Divide and Conquer: Heterogeneous Noise Integration for Diffusion-based Adversarial Purification

Existing diffusion-based purification methods aim to disrupt adversarial perturbations by introducing a certain amount of noise through a forward diffusion process, followed by a reverse process to recover clean examples. However, this approach is fundamentally flawed: the uniform operation of the forward process across all pixels compromises normal pixels while attempting to combat adversarial perturbations, resulting in the target model producing incorrect predictions. Simply relying on low-intensity noise is insufficient for effective defense. To address this critical issue, we implement a heterogeneous purification strategy grounded in the interpretability of neural networks. Our method decisively applies higher-intensity noise to specific pixels that the target model focuses on while the remaining pixels are subjected to only low-intensity noise. This requirement motivates us to redesign the sampling process of the diffusion model, allowing for the effective removal of varying noise levels. Furthermore, to evaluate our method against strong adaptative attack, our proposed method sharply reduces time cost and memory usage through a single-step resampling. The empirical evidence from extensive experiments across three datasets demonstrates that our method outperforms most current adversarial training and purification techniques by a substantial margin.

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_preliminary.tex <==
\section{Preliminary}



\subsection{Diffusion Model}
Diffusion models \cite{DDPM,ImprovedDDPM,Score} are a type of generative model capable of producing high-quality images. They operate through two main processes: the forward process, which converts an image into noise by progressively adding Gaussian noise, and the reverse process, which reconstructs the image from the noise by incrementally removing the noise. The length of both processes is $T$.\\
\textbf{The Diffusion Process.}\quad The diffusion process is a Markov process that gradually adds noise to a clean image until it approaches Gaussian noise. The forward process involves $T$ steps. Resulting in $x_1,x_2,...,x_T$. Due to the Markov property, each step $t$ is only related to the previous step $t-1$.
\begin{equation}
\begin{aligned}
    q(x_t|x_{t-1})&=\mathcal{N}(x_t;\sqrt{1-\beta_t}x_{t-1},\beta_t\textbf{I})\\
    q(x_{1:T}|x_0)&=\prod\limits_{t=1}^T q(x_t|x_{t-1})
\end{aligned}
\end{equation}
where $\beta_t$ is hyperparameter. With $\alpha_t=1-\beta_t$ and $\overline{\alpha}_t=\prod\limits_{s=1}^t \alpha_s$, any step $t$ can be rewritten as one direct sample from
\begin{equation}
    q(x_t|x_0) = \mathcal{N}(x_t;\sqrt{\overline{\alpha}_t}x_0,(1-\overline{\alpha}_t)\textbf{I})
\end{equation}
\textbf{The Reverse Process.} \quad The reverse process is a Markov process that predicts and eliminates the noise added in the diffusion process. Let $x_T\sim\mathcal{N}(0,\textbf{I})$. The reverse process from
latent $x_T$to clean data $x_0$ is defined as
\begin{equation}
\begin{aligned}
    p_{\theta}(x_{t-1}|x_t) &= \mathcal{N}(x_{t-1};\mu_{\theta}(x_t,t),\sigma_t^2\textbf{I})\\
    p_{\theta}(x_{0:T})&=p(x_T)\prod\limits_{t=1}^Tp_{\theta}(x_{t-1}|x_t)
\end{aligned}
\end{equation}
The mean $\mu_{\theta}$  is a neural network parameterized by $\theta$, and the variance $\sigma_t^2$ can be either time step dependent constants \cite{DDPM} or learned by a neural network \cite{ImprovedDDPM}.



\subsection{Activation-based Attention Map}
Activation-based attention map operates by utilizing the activation output of the network's \( m \)-th layer, denoted as \( A_m \in \mathbb{R}^{C_m \times H_m \times W_m} \), where \( C_m \), \( H_m \), and \( W_m \) stand for the number of channels, height, and width, respectively. Let \( M \) be the total number of layers in the network. The process of generating an attention map involves defining a mapping function \( G: \mathbb{R}^{C_m \times H_m \times W_m} \to \mathbb{R}^{H_m \times W_m} \). The magnitude of each value in this attention map signifies its relevance to the final result. Thus, the construction of this mapping relies on computing statistical values across the channel dimension.
More concretely, three types of operations can be applied to formulate the mapping function:
$\mathcal{G}_{\text{sum}}(A_m) = \sum_{i=1}^{C_m} |A_{mi}|$, $
\mathcal{G}_{\text{sum}}^p(A_m) = \left( \sum_{i=1}^{C_m} |A_{mi}|^p \right)^{\frac{1}{p}}$ and 
$\mathcal{G}_{\text{max}}^p(A_m) = \max_{i=1, \dots, C_m} |A_{mi}|^p
$.
Here, $p>1$ and $A_{mi}$ denotes the $i-$th slice of $A_m$ in the channel dimension.

==> sec/4_method.tex <==

\section{Methodology}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\textwidth]{sec/images/attribution_version2.png}
%     \caption{}
%     \label{attribution}
% \end{figure}

% \subsection{Preliminary}
% Activation-based attention map operates by utilizing the activation output of the network's \( m \)-th layer, denoted as \( A_m \in \mathbb{R}^{C_m \times H_m \times W_m} \), where \( C_m \), \( H_m \), and \( W_m \) stand for the number of channels, height, and width, respectively. Let \( M \) be the total number of layers in the network. The process of generating an attention map involves defining a mapping function \( G: \mathbb{R}^{C_m \times H_m \times W_m} \to \mathbb{R}^{H_m \times W_m} \). The magnitude of each value in this attention map signifies its relevance to the final result. Thus, the construction of this mapping relies on computing statistical values across the channel dimension.
% More concretely, three types of operations can be applied to formulate the mapping function:
% Gsum(Am)=∑Cmi=1|Ami|\mathcal{G}_{\text{sum}}(A_m) = \sum_{i=1}^{C_m} |A_{mi}|, $
% \mathcal{G}_{\text{sum}}^p(A_m) = \left( \sum_{i=1}^{C_m} |A_{mi}|^p \right)^{\frac{1}{p}}$ and 
% $\mathcal{G}_{\text{max}}^p(A_m) = \max_{i=1, \dots, C_m} |A_{mi}|^p
% $.
% Here, p>1p>1 and AmiA_{mi} denotes the i−i-th slice of AmA_m in the channel dimension.

% Given an example $(\boldsymbol{x}, \boldsymbol{y})$, an adversary can create a small perturbation to generate an adversarial example $\boldsymbol{x}_{\text{adv}}$ such that the classifier $\boldsymbol{f}$ makes an incorrect prediction: $\boldsymbol{y} \neq \boldsymbol{f}(\boldsymbol{x}_{\text{adv}})$. Existing diffusion-based purification methods obtain a noisy image $\boldsymbol{x}(t)$ at timestep $t$ through the forward process and then recover the clean (or purified) image $\hat{\boldsymbol{x}}$ through the reverse process. And we hope $\boldsymbol{f}(\hat{\boldsymbol{x}}) = \boldsymbol{f}(\boldsymbol{x})$. From the theoretical analysis of \cite{diffpure}, we can find that the timestep $t$ should satisfy: 1) $t$ should be large enough to eliminate perturbations. 2) $t$ should be small enough that $\hat{\boldsymbol{x}}$ still maintains semantic consistency with $\boldsymbol{x}$. We find that these two objectives are contradictory. Therefore, we need to adopt a new forward process to balance both of these objectives.
When given an example (\(\boldsymbol{x}, \boldsymbol{y}\)), an adversary can create a small perturbation to generate an adversarial example \(\boldsymbol{x}_{\text{adv}}\) that leads the classifier \(\boldsymbol{f}\) to make an incorrect prediction: \(\boldsymbol{y} \neq \boldsymbol{f}(\boldsymbol{x}_{\text{adv}})\). Existing diffusion-based purification methods obtain a noisy image \(\boldsymbol{x}(t)\) at timestep \(t\) through the forward process, and then recover the clean (or purified) image \(\boldsymbol{\hat{x}}_t\) through the reverse process. \textcolor{red}{The timestep \(t\) is crucial, as it is positively correlated with the strength of the additive noise from the forward process.} The ultimate goal of purification is to ensure that \(\boldsymbol{f}(\boldsymbol{\hat{x}}_t) = \boldsymbol{f}(\boldsymbol{x}) \neq \boldsymbol{f}(\boldsymbol{x}_{\text{adv}})\). The theoretical analysis from \cite{diffpure} indicates that the timestep \(t\) should meet two criteria: 1) it should be sufficiently \textbf{\textit{large}} to eliminate the perturbations in \(\boldsymbol{x}_{\text{adv}}\), and 2) it should be sufficiently \textbf{\textit{small}} to maintain semantic consistency with \(\boldsymbol{x}\). This contradiction motivates us to develop a new forward process that balances these two objectives.

\textcolor{red}{General evasion attack methods, such as PGD \cite{PGD} and FGSM \cite{RFGSM}, generate additive adversarial perturbations by maximizing the loss function of the target model under specific constraints. This suggests that the adversarial perturbation is likely to be concentrated in areas that are particularly important to the target model}\footnote{\red{tell something about the visualization results.}}. Additionally, attention maps encode the spatial regions of an input that the network focuses on \textcolor{red}{ when making decisions \cite{saliency, grad-cam++, grad-cam, feature-attribution, attribution, paying}.} Therefore, the proposed method introduces high-intensity noise to eliminate adversarial perturbations in areas of \textcolor{red}{ high attention} while applying low-intensity noise to the remaining regions, thereby preserving semantic information as much as possible.
% \begin{enumerate}
%     \item tt should be large enough to \textbf{eliminate perturbations} of \boldsymbol{x}_{adv}\boldsymbol{x}_{adv},
%     \item tt should be small enough to maintain \textbf{semantic consistency} with \boldsymbol{x}\boldsymbol{x}.
% \end{enumerate}
% Such a contradictory inspires us to develop a new forward process to balance these two objectives.
%DKL(pt∥qt)≤ϵD_{KL}(p_{t} \parallel q_{t}) \leq \epsilon, 
% tt should be large enough to \textbf{eliminate perturbations} of \boldsymbol{x}_{adv}\boldsymbol{x}_{adv}. 2) 
%||\boldsymbol{\hat{x}}(0)-\boldsymbol{x} ||\leq ||\boldsymbol{\delta}_{adv}|| + g(t)||\boldsymbol{\hat{x}}(0)-\boldsymbol{x} ||\leq ||\boldsymbol{\delta}_{adv}|| + g(t), 
% tt should be small enough to maintain \textbf{semantic consistency} with \boldsymbol{x}\boldsymbol{x}. 
%\textit{Can we eliminate adversarial perturbations while still preserving most of the semantic information of the image?} 
\\



% attention, a set of maps, encodes the spatial regions of input that the network focuses on when making decisions \cite{saliency,grad-cam++,grad-cam,feature-attribution,attribution,paying}. Meanwhile,  \textcolor{blue}{These suggests that, for an adversarial example, adversarial perturbations in the regions where the classifier focuses on contribute to causing the classifier to make incorrect predictions.} Therefore, we propose that we introduce high-intensity noise to eliminate adversarial perturbations of the regions with more attention and applying low-intensity noise to the remaining area to preserve as much semantic information as possible. 
% Among various interpretability methods \cite{saliency,grad-cam++,grad-cam,feature-attribution,attribution,paying} for neural networks, 

% the attention maps for each layer of the target classifier can be obtained with a single forward propagation, without the need for additional supervision information. Attention is a set of spatial maps. It is primarily used to encode the input spatial regions that the network focuses on most when making output decisions, such as in image classification. 
%In the ???????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{forward}, we introduce how we applying different level noise with the attention mask we construct. In the ???????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{Sampling Method}, we introduce how we recover the clean image with heterogeneous denoising process.

\subsection{Heterogeneous Forward Process}
\label{forward}
% \textbf{Activation-based Attention Map.} The activation of the network's \( m \)-th layer is a tensor, denoted as \( A_m \in \mathbb{R}^{C_m \times H_m \times W_m} \), where \( C_m \), \( H_m \), and \( W_m \) stand for the number of channels, height, and width, respectively. 
% %Let \( M \) be the total number of layers in the network. 
% To obtain an attention map involves defining a mapping function \( G: \mathbb{R}^{C_m \times H_m \times W_m} \to \mathbb{R}^{H_m \times W_m} \). The magnitude of each value in this attention map reflects its relevance to the final result. Thus, this mapping relies on computing statistical values across the channel dimension.
% % More concretely, three types of operations can be applied to formulate the mapping function:
% % Gsum(Am)=∑Cmi=1|Ami|\mathcal{G}_{\text{sum}}(A_m) = \sum_{i=1}^{C_m} |A_{mi}|, $
% % \mathcal{G}_{\text{sum}}^p(A_m) = \left( \sum_{i=1}^{C_m} |A_{mi}|^p \right)^{\frac{1}{p}}$ and 
% % $\mathcal{G}_{\text{max}}^p(A_m) = \max_{i=1, \dots, C_m} |A_{mi}|^p
% % $.
% % Here, p>1p>1 and AmiA_{mi} denotes the i−i-th slice of AmA_m in the channel dimension.
% Attention maps are always defined at various layers of the network to capture low, mid, and high-level representation information, which reflects how the neural network assigns weights to different regions of an image \cite{paying}. \textcolor{red}{Here, we adopt Gpsum(Am)\mathcal{G}_{\text{sum}}^p(A_m) as the attention function and set p=2p=2 because \cite{lane} found it to be the most effective in their results.}
When purifying the adversarial example $\boldsymbol{x}_{adv}$ with the diffusion model, \textcolor{red}{we treat $\boldsymbol{x}_{adv}$ as a starting point of the noisy images sequence $\{\boldsymbol{x}(t)\ |\ \boldsymbol{x}(0) = \boldsymbol{x}_{adv}\}$.} Choose two noisy images of this sequence with different timestep $\boldsymbol{x}(t_l),\boldsymbol{x}(t_b), t_l > t_s$ , we have
\begin{subequations}
    \label{eq:forward}
    \begin{align}
        \boldsymbol{x}(t_l) &= \sqrt{\overline{\alpha}(t_l)}\cdot \boldsymbol{x}(0) + \sqrt{1 - \overline{\alpha}(t_l)}\cdot \boldsymbol{\epsilon}\label{x(t_l)},\\
        \boldsymbol{x}(t_s) &= \sqrt{\overline{\alpha}(t_s)}\cdot \boldsymbol{x}(0) + \sqrt{1 - \overline{\alpha}(t_s)}\cdot \boldsymbol{\epsilon}\label{x(t_s)},
\end{align}
\end{subequations}
where $\{\sqrt{\overline{\alpha}(t)}\}$ is a series of given parameters and $\boldsymbol{\epsilon} \sim \mathcal{N}(0, \boldsymbol{I})$.
% \textcolor{red}{where ¯α(⋅)\overline{\alpha}(\cdot) is XXXXXXXXXXXX, and ϵ\epsilon is XXXXXXXXXX.} 
% Then the clean images \boldsymbol{\hat{x}}_{t_l}\boldsymbol{\hat{x}}_{t_l} and \boldsymbol{\hat{x}}_{t_s}\boldsymbol{\hat{x}}_{t_s} from eqref{x(t_s)} are obtained through the normal reverse process \cite{diffpure,DDPM}, respectively. For samller timestep t_st_s, the recovered image \boldsymbol{\hat{x}}_{t_b}\boldsymbol{\hat{x}}_{t_b} still maintain part of adversarial perturbations and will result in  \boldsymbol{f}(\boldsymbol{x}_{adv}) = \boldsymbol{f}(\boldsymbol{\hat{x}}_{t_s}) \neq \boldsymbol{f}(\boldsymbol{x}) \boldsymbol{f}(\boldsymbol{x}_{adv}) = \boldsymbol{f}(\boldsymbol{\hat{x}}_{t_s}) \neq \boldsymbol{f}(\boldsymbol{x}). And for larger timestep t_at_a, the clean image \boldsymbol{\hat{x}}_{t_a}\boldsymbol{\hat{x}}_{t_a} will lose original semantic information, causing \boldsymbol{f}(\boldsymbol{x}_{adv}) \neq \boldsymbol{f}(\boldsymbol{\hat{x}}_{t_a}) \neq \boldsymbol{f}(\boldsymbol{x})\boldsymbol{f}(\boldsymbol{x}_{adv}) \neq \boldsymbol{f}(\boldsymbol{\hat{x}}_{t_a}) \neq \boldsymbol{f}(\boldsymbol{x}). To diffuse the different areas of the images with different timesteps, we introduce how we construct an attention mask.
\textcolor{red}{The clean images \(\boldsymbol{\hat{x}}_{t_l}\) and \(\boldsymbol{\hat{x}}_{t_s}\), obtained from \eqref{x(t_l)} and \eqref{x(t_s)} respectively, are processed through the subsequent reverse process \cite{diffpure,DDPM}.} For the smaller timestep \(t_s\), the recovered image \(\boldsymbol{\hat{x}}_{t_s}\) retains certain adversarial perturbation, resulting in \(\boldsymbol{f}(\boldsymbol{x}_{adv}) = \boldsymbol{f}(\boldsymbol{\hat{x}}_{t_s}) \neq \boldsymbol{f}(\boldsymbol{x})\). Conversely, at the larger timestep \(t_l\), the clean image \(\boldsymbol{\hat{x}}_{t_l}\) loses critical semantic information, leading to \(\boldsymbol{f}(\boldsymbol{x}_{adv}) \neq \boldsymbol{f}(\boldsymbol{\hat{x}}_{t_l}) \neq \boldsymbol{f}(\boldsymbol{x})\). To effectively aggregate the differing impacts on various regions of the images at distinct timesteps, we construct an attention mask to integrate \eqref{x(t_l)} and \eqref{x(t_s)}.
% To balance balance between preserving
% semantic information and eliminating adversarial perturbations, we propose that we can diffuse different regions of the image \boldsymbol{x}_{adv}\boldsymbol{x}_{adv} with different timestep t_at_a and t_bt_b. This motivates us to construct an attention mask based on the assignment of the attention weights of the classifier. First, we introduce how we construct the attention mask and then we propose our forward process. 

Consider a neural network that consists of $M$ blocks (\textit{e.g.} ResNet-50 \cite{resnet} consists of $4$ blocks). For $m$-th block, we extract the output of the last activation function (\textit{e.g.} Relu \cite{relu} or Swish \cite{swish}) as follows: 
\begin{equation}
    % \mathcal{G}_m = \mathcal{G}_{\text{sum}}^p(A_m) = \left( \sum_{i=1}^{C_m} |A_{mi}|^p \right)^{\frac{1}{p}}, m\in[M],
    \boldsymbol{G}_m  = \left( \sum_{i=1}^{C_m} |\boldsymbol{A}_{mi}|^p \right)^{\frac{1}{p}}\in \mathbb{R}^{H_m \times W_m}, m\in[M],
\end{equation}
where $p\in\mathbb{N}$, $C_m, H_m, W_m$ are the dimension of channels, height, and width respectively, $\boldsymbol{A}_m$ denotes the activation of \( m \)-th block and $\boldsymbol{A}_{mi}$ denotes the $i$-th slice of $\boldsymbol{A}_m$ along the channel dimension. Then we apply interpolation techniques to ensure it matches the original image size. By upsampling $\boldsymbol{G}_m$ with bilinear function $\text{Bi}(\cdot)$, we obtain attention map of $m$-th block:
\begin{equation}
    \text{AM}_m = \phi(\text{Bi}(\boldsymbol{G}_m)),
\end{equation}
where $\phi(\cdot)$ is the spatial softmax operation. Moreover, we build the attention mask with all attention maps $\{\text{AM}_m\}$:
%It is noteworthy that shallow attention maps primarily provide low-level feature information, while deep attention maps offer middle and high-level semantic information. 
% Once the attention maps {AMm}\{AM_m\} of the network at different levels for the input image, we can utilize these attention maps to construct attention mask for dividing different regions to apply varying intensities of noise. Shallow attention maps primarily provide low-level feature information, while deep attention maps offer mid- and high-level semantic information. Additionally, ablation study {Ablation Study} demonstrate that removing any block will impact performance.
% Therefore, We choose to utlize all-level attention maps to construct the attention mask as follows:
\begin{equation}
    \label{attention-mask}
    % \mathcal{M} = \max\big\{\mathbb{I}[AM_1>\tau]\cup\dots\cup\mathbb{I}[AM_M>\tau]\big\},
    \mathcal{M} = \bigcup_{m=1}^M \mathbb{I}\ [\text{AM}_m>\tau]
\end{equation}
where $\mathbb{I}\ [\cdot]$ is the Iverson bracket and $\tau$ is the threshold to distinguish important and ordinary regions. With the attention mask $\mathcal{M}$ and two noisy images from Eq.\eqref{eq:forward}, $\boldsymbol{x}(t_s),\boldsymbol{x}(t_l), t_s<t_l$, the result of the proposed heterogeneous forward process is 
\begin{equation}
    \label{x_a&b}
    \boldsymbol{x}(t_l,t_s) = \boldsymbol{x}(t_l) \odot \mathcal{M} + \boldsymbol{x}(t_s) \odot (1-\mathcal{M}),
\end{equation}
where $\odot$ is the Hadamard product. 
% Suppose we obtain the attention mask $\mathcal{M}$ using \eqref{attention-mask} and the noisy image $\boldsymbol{\hat{x}}_{t_s}$ and $\boldsymbol{\hat{x}}_{t_l}$ from \eqref{x(t_s)} and \eqref{x(t_l)}, respectively, we diffuse different regions of the image with $\mathcal{M}$ as follows:
% \begin{equation}
%     \label{x_a&b}
%     \boldsymbol{x}(t_a,t_b) = \boldsymbol{x}(t_a) \odot \mathcal{M} + \boldsymbol{x}(t_b) \odot (1-\mathcal{M}).
% \end{equation}
\subsection{Heterogeneous Denoising Process}
\label{Denoising}
% We aim to remove noise of varying intensities from an image in order to restore its original pixel values with the diffusion model. Note that we don't need to retrain the diffusion model, we can achieve this goal simply by improving the sampling process. Given an adversarial example xadvx_{adv} at
% timestep $t=0$, \textit{i.e.} $x(0) = x_{adv}$ and the attention mask $M$ using \eqref{mask}. We diffuse different regions of the image based on the attention mask, where regions with a mask value of $1$ diffuse for timestep $t_a$ and the remain regions for $t_n$, with  $t_a>t_n$. Here we can get two noisy images with different intensity of noise:
% Given an adversarial example $\boldsymbol{x}_{adv}$ at
% timestep $t=0$, \textit{i.e.} $\boldsymbol{x}(0) = \boldsymbol{x}_{adv}$ and two timestep $t_a$ and $t_b$ with $t_a > t_b$. We get the noisy images as follows:
% \begin{subequations}
% \begin{align}
%     \boldsymbol{x}(t_b) &= \sqrt{\overline{\alpha}(t_b)} \boldsymbol{x}_{adv} + \sqrt{1 - \overline{\alpha}(t_b)}\boldsymbol{ \epsilon}\label{x(t_b)}\\
% \boldsymbol{x}(t_a) &= \sqrt{\overline{\alpha}(t_a)} \boldsymbol{x}_{adv} + \sqrt{1 - \overline{\alpha}(t_a)}\boldsymbol{ \epsilon}\label{x(t_a)} 
% \end{align}
% \end{subequations}
% Then we get the clean images $x_{t_a}$ and $x_{t_b}$ through the reverse process, respectively. The image $x_{t_b}$ still maintain part of adversarial perturbations and will result in $ \boldsymbol{f}(\boldsymbol{x}+\boldsymbol{\delta}_{adv}) = \boldsymbol{f}(x_{t_b}) \neq \boldsymbol{f}(x)$. And for image $x_{t_a}$ will lose original semantic, therefore $\boldsymbol{f}(\boldsymbol{x}+\boldsymbol{\delta}_{adv}) \neq \boldsymbol{f}(x_{t_a}) \neq \boldsymbol{f}(x)$. \\
% Suppose we get the attention mask $\mathcal{M}$ using \ref{Attention Mask}. To  eliminate perturbations and maintains semantic consistency, we diffuse different regions of the image based on the attention mask $\mathcal{M}$ with noisy image from \eqref{x(t_a)} and \eqref{x(t_b)} as follows:
% \begin{equation}
%     \label{x_a&b}
%     \boldsymbol{x}(t_a,t_b) = \boldsymbol{x}(t_a) \odot \mathcal{M} + \boldsymbol{x}(t_b) \odot (1-\mathcal{M})
% \end{equation}
% \textcolor{red}{The selection of $t_a$ and $t_b$ is discussed in detail in Section \ref{Ablation Study}}. 
% How do you remove noise from varying intensities from different regions of an image? 
Given a noisy image generated by the proposed heterogeneous forward process like \eqref{x_a&b}, \textcolor{red}{the standard reverse process can't handle $\boldsymbol{x}(t_l,t_s)$ due to the different noise intensities of $\boldsymbol{x}(t_l)$ and $\boldsymbol{x}(t_s)$. It is known that the standard denoising of the diffusion model is a descending process according to $t$.} Consequently, a two-stage reverse process is designed to implement heterogeneous denoising. \textcolor{red}{In the early stages, we try to eliminate high-intensity noise in the region indicated by $\mathcal{M}$, while the late phases focus on processing the other areas.} 
% More specifically, for the current timestep $t\in[1,t_l]$, we utilize different strategies.
% \textcolor{blue}{The noisy image \eqref{x_a&b} via our forward process contains different intensity noise. We should first remove high-intensity local noise, then eliminate low-intensity noise. When removing high-intensity noise, low-intensity noise provides supervision for the removal of high-intensity noise until the noise intensity in the image becomes consistent.} Therefore, to recover the clean image, we design a two-stage denoising process. For the current timestep $t$, we consider the following two cases:\\
% \begin{equation}
%     x(t_a) = \sqrt{\alpha(t_a)} x_{adv} + \sqrt{1 - \alpha(t_a)} \epsilon
% \end{equation}
% \begin{equation}
%     x(t_n) = \sqrt{\alpha(t_n)} x_{adv} + \sqrt{1 - \alpha(t_n)} \epsilon
% \end{equation}
% Due to varying noise intensities in different regions of the image, we need to consider two scenarios when performing reverse sampling using the diffusion model:\\
\begin{itemize}
    \item \textbf{Stage I. } When $t\in[t_s, t_l)$, the pixels inside $\mathcal{M}$ should be predicted from the previous results at $t+1$:
    \begin{equation}
        \label{unknown}
        \begin{aligned}
            \boldsymbol{\tilde{x}}(t)\sim\mathcal{N}\big(\boldsymbol{\mu}_{\boldsymbol{\theta}}(\boldsymbol{\tilde{x}}(t+1)), \boldsymbol{\Sigma}_{\boldsymbol{\theta}}(\boldsymbol{\tilde{x}}(t+1))\big),
        \end{aligned}
    \end{equation}
    \textcolor{red}{where $\boldsymbol{\mu}_{\boldsymbol{\theta}}(\cdot)$ is the mean which is calculated via the noise $\epsilon_{\theta}$ predicted by diffusion model, and $\boldsymbol{\Sigma}_{\boldsymbol{\theta}}(\cdot)$ is variance.} Meanwhile, the pixels outside $\mathcal{M}$ can be obtained by forward process\footnote{\red{tell something about why not store all images but compute this step by step.}} like \eqref{eq:forward}:
    \begin{equation}
        \label{known}
        \boldsymbol{\breve{x}}(t) = \sqrt{\overline{\alpha}(t)}\cdot\boldsymbol{x}(0) + \sqrt{1-\overline{\alpha}(t)}\cdot\boldsymbol{\epsilon}.
    \end{equation}
    Then we combine $\boldsymbol{\tilde{x}}(t)$ and $\boldsymbol{\breve{x}}(t)$ together with $M$ to get the clean image $\boldsymbol{\hat{x}}(t)$ at $t$:
    \begin{equation}
        \label{merge}
        \boldsymbol{\hat{x}}(t) = \mathcal{M}\odot\boldsymbol{\tilde{x}}(t) + (1 -\mathcal{M}) \odot\boldsymbol{\breve{x}}(t).
    \end{equation}
    Notably, to keep $\boldsymbol{\hat{x}}(t)$ as close as possible to the natural picture \cite{repaint}, the reverse process could execute \eqref{unknown} and \eqref{known} many times before aggregation. The existing diffusion-based purification methods, which only handle homogeneous noise, also adopt this strategy. However, this brings a huge overhead in terms of time and space. We greatly reduce such overhead by improving \eqref{known} while maintaining the denoising effect in Sec. \ref{Time and Space Efficiency}. Such improvement helps the proposed purification method resist the strong adaptive attack. 
    % Therefore, this case can be viewed as an inpainting problem \cite{repaint}.
    \item \textbf{Stage II. } As $t\in[1,t_s)$, the intensities of noise inside and outside $M$ are same. Therefore, we can proceed with the standard sampling process of the diffusion model to get $\boldsymbol{\hat{x}}(t)$:
    \begin{equation}
        \label{reverse}
            \begin{aligned}
            \boldsymbol{x}(t)\sim\mathcal{N}(\boldsymbol{\mu}_{\boldsymbol{\theta}}(\boldsymbol{\hat{x}}(t+1)), \boldsymbol{\Sigma}_{\boldsymbol{\theta}}(\boldsymbol{\hat{x}}(t+1)).
    \end{aligned}
\end{equation}
\end{itemize}
The whole denoising process is listed as Algorithm \ref{sampling-argotithm}.

% \textbf{Case 1 ($\boldsymbol{t_s<t<t_l}$)}\quad When the current timestep $t$ lies between $t_a$ and $t_b$. For the pixels inside the attention mask $\mathcal{M}$, they should be predicted from the previous timestep $t+1$. But for the pixels outside the attention mask $\mathcal{M}$, they can be obtained by further adding noise forward from \eqref{x_a&b}. Therefore, this case can be viewed as a inpainting problem \cite{repaint}.  
% For the image regions outside the attention mask $\mathcal{M}$, since only the forward process is involved. Therefore, we can get the pixels value of these regions at timestep $t$ equivalently as follows:
% \begin{equation}
% \label{known}
%     \boldsymbol{x}(t)^{known} = \sqrt{\overline{\alpha}(t)} \boldsymbol{x}_{adv} + \sqrt{1 - \overline{\alpha}(t)}\boldsymbol{ \epsilon}.
% \end{equation}
%  For the image regions within the attention mask, the pixels value of these regions at timestep $t$ should be predicted by diffusion model:
% \begin{equation}
%     \label{unknown}
%     \begin{aligned}
%         & & &\ \ \boldsymbol{x}(t)^{unknown}\\
%         & &\sim&\ \ \mathcal{N}(\mu_\theta(\boldsymbol{x}(t+1), t+1), \Sigma_\theta(\boldsymbol{x}(t+1), t+1)),
%     \end{aligned}
% \end{equation}
% where $\theta$ is the parameters of the diffusion model. Then we combine $x(t)^{known}$ and $x(t)^{unknown}$ together based on the attention mask $M$ to get the  $\boldsymbol{x}(t)$ at timestep $t$:
% \begin{equation}
% \label{merge}
% \boldsymbol{x}(t) = \mathcal{M} \odot \boldsymbol{x}(t)^{known} + (1 - \mathcal{M}) \odot \boldsymbol{x}(t)^{unknown},
% \end{equation}
% where $\odot$ is hadamard product. We can remove the localized strong noise through the case 1.\\
% \textbf{Case 2 ($\boldsymbol{t<t_s}$)}\quad When the current timestep $t$ is less than $t_b$, since the noise intensity is the same both inside and outside the attention mask. Therefore, the attention mask $\mathcal{M}$ is no longer needed. At this point, we can proceed with the standard sampling process of the diffusion model. We can get $x(t)$ predicted from the previous timestep $x(t+1)$ as follows:
% \begin{equation}
%     \label{reverse}
%     \begin{aligned}
%         & & &\ \ \boldsymbol{x}(t)\\
%         & &\sim&\ \ \mathcal{N}(\mu_\theta(\boldsymbol{x}(t+1), t+1), \Sigma_\theta(\boldsymbol{x}(t+1), t+1)).
%     \end{aligned}
% \end{equation}
% Following the case 2, we will eliminate global weak noise and get the clean image. The complete algorithm process can be found in the Algorithm \ref{sampling-argotithm}.

\begin{algorithm}[htbp]
\caption{Heterogeneous Denoising Process}
\label{sampling-argotithm}
\begin{algorithmic}
\REQUIRE Sample $x_0$, Attention Mask $\mathcal{M}$, Forward Steps $t_s,t_l$, Diffusion model parameters $\theta$.

% \STATE Inital Timestep Schedule $ \{\tau_0, \tau_1, \dots, \tau_s \}$, where $\tau_s=T_b$ 

\FOR{$t=t_l,...,1$}
\STATE \textbf{if} $t<t_s$ \textbf{then} \COMMENT{Case 2} 

\STATE\quad $z \sim \mathcal{N}(0, \mathbf{I}) \text{ if }  t > 1, \text{ else } z = 0$ 
\STATE\quad $x_{t-1} = \frac{1}{\sqrt{\alpha_t}} \left( x_t - \frac{\beta_t}{\sqrt{1-\bar{\alpha}_t}} \epsilon_\theta(x_t, t) \right) + \sigma_t z$ 
% \ELSIF{$T_b \leq t \leq T_a$}
\STATE\textbf{else if} $t_s \leq t \leq t_l$ \textbf{then} 
\COMMENT{Case 1}
\STATE\quad $\epsilon \sim \mathcal{N}(0, \mathbf{I}) \text{ if } t > 1, \text{ else } \epsilon = 0$
\STATE\quad$x_{t-1}^{known} = \sqrt{\overline{\alpha}_{t-1}} x_0 + \sqrt{1-\overline{\alpha}_{t-1}}\epsilon$
\STATE\quad $z \sim \mathcal{N}(0, \mathbf{I}) \text{ if }  t > 1, \text{ else } z = 0$
\STATE\quad $x_{t-1}^{unknown} = \frac{1}{\sqrt{\alpha_t}} \left( x_t - \frac{\beta_t}{\sqrt{1-\bar{\alpha}_t}} \epsilon_\theta(x_t, t) \right) + \sigma_t z$
\STATE\quad$x_{t-1} = \mathcal{M} \odot x_{t-1}^{known} + (1 - \mathcal{M}) \odot x_{t-1}^{unknown}$


% \ENDIF
\STATE\textbf{for} $u=1,2,...U$ \textbf{do} \COMMENT{Resampling}
\STATE\quad $z \sim \mathcal{N}(0, \mathbf{I}) \text{ if }  t > 1, \text{ else } z = 0$
\STATE\quad$x_{t-1+u} = \sqrt{\alpha_{t-1+u}} x_{t+u-2} + \sqrt{1 - \alpha_{t-1+u}} z$
\STATE\textbf{end for}

% \STATE $z \sim \mathcal{N}(0, \mathbf{I}) \text{ if }  t > 1, \text{ else } z = 0$
\STATE get $x_{t-1}$ using \eqref{ddim} 
\ENDFOR

\end{algorithmic}
\end{algorithm}

\section{Adaptive Attack to Diffusion Purification }
\label{Time and Space Efficiency} 
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.5\textwidth]{sec/images/repaint&ours.png}
%     \caption{Our method maintains semantic consistency between the masked areas and the surrounding pixel values when $U=10$. Note that no matter what $U$ is, our method requires only one additional call to the diffusion model. }
%     \label{efficiency}
% \end{figure}
When directly applying the method described in \ref{Denoising}, we obsevere the same phenomenon as \cite{repaint} that although the region recovered in the case 2 matches the texture of the neighboring region, it is semantically incorrect.
We can observe this phenomenon in the Figure \ref{efficiency}. \cite{repaint} addresses this issue via muti-step resampling by diffusing the output $\boldsymbol{x}(t)$ back to $\boldsymbol{x}(t+1)$: 
\begin{equation} 
\label{back}
\boldsymbol{x}(t+1) = \sqrt{\alpha(t)} \boldsymbol{x}(t) + \sqrt{1 - \alpha(t)} \boldsymbol{\epsilon},
\end{equation}
and it is necessary to fully execute \ref{Denoising} again to get $\boldsymbol{x}(t)$. From Figure \ref{efficiency} we can find that this process needs to be repeated $U=20$ times to ensure that the masked region becomes semantically consistent with the surrounding pixels. To evaluate our method against strong adaptive attacks \cite{diffpure}, it is necessary to compute the full gradient of the whole sampling process to construct adversarial examples. To reduce the time cost and memory usage, we optimized the multi-step resampling into a single resampling process which achieves the same functionality.
%Suppose the denoising steps is $T$, then the GPU memory needs to store the  $U * T$ complete computation graphs of u-net model, which is impossible to compute the full gradient. The key to reducing memory usage during sampling is to avoid frequent calls to the u-net model. \\
\\The intuition behind our improvement is that repeating \eqref{back} and \ref{Denoising} for $U$ times is equivalent to first diffuse $\boldsymbol{x}(t)$ to $\boldsymbol{x}(t+U)$ and then denoise it back to $\boldsymbol{x}(t)$ from $\boldsymbol{x}(t+U)$ in a single step using DDIM \cite{ddim} as follows:
\begin{equation}
\label{ddim}
\begin{aligned}
    x_{t-1} &= \sqrt{\alpha_{t-1}} \left( \frac{\boldsymbol{x}_{t-1+U} - \sqrt{1 - \alpha_{t-1+U}} \epsilon_{\theta}(\boldsymbol{x}_{t-1+U})}{\sqrt{\alpha_{t-1+U}}} \right) \\
    &+ \sqrt{1 - \alpha_{t-1} - \sigma^2_{t-1+U}} \cdot \epsilon_{\theta}(\boldsymbol{x}_{t-1+U}) + \sigma_{t-1+U} z.
\end{aligned}
\end{equation}
From the bottom panel of Figure \ref{efficiency}, we find that our method can also achieve semantically incorrect when $U=10$. This means that at each timestep, we only need to invoke the diffusion model an additional time. Therefore, the GPU memory needs to store the  $2 * T$ complete computation graphs of u-net model which enables the computation of gradient of our method on consumer-grade GPU with only 24G memory. Also the time cost is also greatly reduced. The analysis of time cost and memory usage can refer to Section \ref{Space and Time}.
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\textwidth]{sec/images/repaint&ours.png}
    \caption{Our method maintains semantic consistency between the masked areas and the surrounding pixel values when $U=10$. Note that no matter what $U$ is, our method requires only one additional call to the diffusion model. }
    \label{efficiency}
\end{figure}




% \begin{algorithm}[htbp]
% \caption{Sampling Method}
% \label{algorithm-1}
% \begin{algorithmic}
% \REQUIRE Sample $x_0$, Attention Mask $m$, Forward Steps $T_a,T_b$, Diffusion model parameters $\theta$.

% \STATE Inital Timestep Schedule $ \{\tau_0, \tau_1, \dots, \tau_s \}$, where $\tau_s=T_b$ 

% \FOR{$i=s,...,1$}
% \STATE $\epsilon \sim \mathcal{N}(0, \mathbf{I}) \text{ if } \tau_i > 1, \text{ else } \epsilon = 0$

% \STATE$X_{\tau_{i-1}}^{known} = \sqrt{\overline{\alpha}_{\tau{i-1}}} x_0 + \sqrt{1-\overline{\alpha}_{\tau_{i-1}}}\epsilon$
% \IF{$T_b \leq \tau_{i-1} < T_a$}
% \STATE $z \sim \mathcal{N}(0, \mathbf{I}) \text{ if }  \tau_i > 1, \text{ else } \mathbf{z} = 0$
% \STATE $X_{\tau_{i-1}}^{unknown} = \sqrt{\alpha_{\tau_{i-1}}} \left( \frac{\mathbf{x}_{\tau_i} - \sqrt{1 - \alpha_{\tau_i}} \epsilon_{\theta}(\mathbf{x}_{\tau_i})}{\sqrt{\alpha_{\tau_i}}} \right) + \sqrt{1 - \alpha_{\tau_{i-1}} - \sigma^2_{\tau_i}} \cdot \epsilon_{\theta}(\mathbf{x}_{\tau_i}) + \sigma_{\tau_i} \epsilon
% $
% \STATE$x_{\tau_{i-1}} = m \odot x_{\tau_{i-1}}^{known} + (1 - m) \odot x_{\tau_{i-1}}^{unknown}$
% \ELSIF{$\tau_{i-1}<T_b$}
% \STATE $X_{\tau_{i-1}} = \sqrt{\alpha_{\tau_{i-1}}} \left( \frac{\mathbf{x}_{\tau_i} - \sqrt{1 - \alpha_{\tau_i}} \epsilon_{\theta}(\mathbf{x}_{\tau_i})}{\sqrt{\alpha_{\tau_i}}} \right) + \sqrt{1 - \alpha_{\tau_{i-1}} - \sigma^2_{\tau_i}} \cdot \epsilon_{\theta}(\mathbf{x}_{\tau_i}) + \sigma_{\tau_i} \epsilon
% $
% \ENDIF
% \FOR{$u=1,2,...U$}
% \STATE $X_{\tau_{i-1}+u} = \sqrt{\alpha_{\tau_{i-1}+u}} x_{\tau_{i-1}+u-1} + \sqrt{1 - \alpha_{\tau_{i-1}+u}} \epsilon
% $
% \ENDFOR
% \STATE $X_{\tau_{i-1}} = \sqrt{\alpha_{\tau_{i-1}}} \left( \frac{\mathbf{x}_{\tau_i-1+U} - \sqrt{1 - \alpha_{\tau_i-1+U}} \epsilon_{\theta}(\mathbf{x}_{\tau_i-1+U})}{\sqrt{\alpha_{\tau_i-1+U}}} \right) + \sqrt{1 - \alpha_{\tau_{i-1}} - \sigma^2_{\tau_i-1+U}} \cdot \epsilon_{\theta}(\mathbf{x}_{\tau_i-1+U}) + \sigma_{\tau_i-1+U} \epsilon
% $

% \ENDFOR
% \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[H]
% \caption{Adversarial Purification}
% \label{algorithm-1}
% \begin{algorithmic}
% \REQUIRE Sample $x_0$, Attention Mask $m$, Forward Steps $T_a,T_b$, Diffusion model parameters $\theta$.

% \STATE Inital Timestep Schedule $ \{\tau_0, \tau_1, \dots, \tau_s \}$, where $\tau_s=T_b$ 

% \FOR{$i=s,...,1$}
% \STATE $\epsilon \sim \mathcal{N}(0, \mathbf{I}) \text{ if } \tau_i > 1, \text{ else } \epsilon = 0$

% \STATE$X_{\tau_{i-1}}^{known} = \sqrt{\overline{\alpha}_{\tau{i-1}}} x_0 + \sqrt{1-\overline{\alpha}_{\tau_{i-1}}}\epsilon$
% \IF{$T_b \leq \tau_{i-1} < T_a$}
% \STATE $z \sim \mathcal{N}(0, \mathbf{I}) \text{ if }  \tau_i > 1, \text{ else } \mathbf{z} = 0$
% \STATE $X_{\tau_{i-1}}^{unknown} = \sqrt{\alpha_{\tau_{i-1}}} \left( \frac{\mathbf{x}_{\tau_i} - \sqrt{1 - \alpha_{\tau_i}} \epsilon_{\theta}(\mathbf{x}_{\tau_i})}{\sqrt{\alpha_{\tau_i}}} \right) + \sqrt{1 - \alpha_{\tau_{i-1}} - \sigma^2_{\tau_i}} \cdot \epsilon_{\theta}(\mathbf{x}_{\tau_i}) + \sigma_{\tau_i} \epsilon
% $
% \STATE$x_{\tau_{i-1}} = m \odot x_{\tau_{i-1}}^{known} + (1 - m) \odot x_{\tau_{i-1}}^{unknown}$
% \ELSIF{$\tau_{i-1}<T_b$}
% \STATE $X_{\tau_{i-1}} = \sqrt{\alpha_{\tau_{i-1}}} \left( \frac{\mathbf{x}_{\tau_i} - \sqrt{1 - \alpha_{\tau_i}} \epsilon_{\theta}(\mathbf{x}_{\tau_i})}{\sqrt{\alpha_{\tau_i}}} \right) + \sqrt{1 - \alpha_{\tau_{i-1}} - \sigma^2_{\tau_i}} \cdot \epsilon_{\theta}(\mathbf{x}_{\tau_i}) + \sigma_{\tau_i} \epsilon
% $
% \ENDIF
% \FOR{$u=1,2,...U$}
% \STATE $X_{\tau_{i-1}+u} = \sqrt{\alpha_{\tau_{i-1}+u}} x_{\tau_{i-1}+u-1} + \sqrt{1 - \alpha_{\tau_{i-1}+u}} \epsilon
% $
% \ENDFOR
% \STATE $X_{\tau_{i-1}} = \sqrt{\alpha_{\tau_{i-1}}} \left( \frac{\mathbf{x}_{\tau_i-1+U} - \sqrt{1 - \alpha_{\tau_i-1+U}} \epsilon_{\theta}(\mathbf{x}_{\tau_i-1+U})}{\sqrt{\alpha_{\tau_i-1+U}}} \right) + \sqrt{1 - \alpha_{\tau_{i-1}} - \sigma^2_{\tau_i-1+U}} \cdot \epsilon_{\theta}(\mathbf{x}_{\tau_i-1+U}) + \sigma_{\tau_i-1+U} \epsilon
% $

% \ENDFOR
% \end{algorithmic}
% \end{algorithm}

